S-HR-VQVAE: Sequential Hierarchical Residual Learning Vector Quantized Variational Autoencoder for Video Prediction

We address the video prediction task by putting forth a novel model that combines (i) a novel hierarchical residual learning vector quantized variational autoencoder (HR-VQVAE), and (ii) a novel autoregressive spatiotemporal predictive model (AST-PM). We refer to this approach as a sequential hierarchical residual learning vector quantized variational autoencoder (S-HR-VQVAE). By leveraging the intrinsic capabilities of HR-VQVAE at modeling still images with a parsimonious representation, combined with the AST-PM's ability to handle spatiotemporal information, S-HR-VQVAE can better deal with major challenges in video prediction. These include learning spatiotemporal information, handling high dimensional data, combating blurry prediction, and implicit modeling of physical characteristics. Extensive experimental results on four challenging tasks, namely KTH Human Action, TrafficBJ, Human3.6M, and Kitti, demonstrate that our model compares favorably against state-of-the-art video prediction techniques both in quantitative and qualitative evaluations despite a much smaller model size. Finally, we boost S-HR-VQVAE by proposing a novel training method to jointly estimate the HR-VQVAE and AST-PM parameters.

==> figs/psnr_all.tex <==


\begin{tikzpicture}
      \begin{axis}[
        ybar,
        width=12cm,
        height=6.5cm,
        symbolic x coords={ConvLSTM, DFN, CDNA, DrNet, PredRNN, McNet, MsNet, fRNN, PredRNN++, E3D-LSTM, Conv-TT-LSTM, LMC-Memory, V-3D-ConvLSTM, R-ST-ConvLSTM, PredRNN-V2, VPTR*, 3-LayerHVP},
        xtick={ConvLSTM, DFN, CDNA, DrNet, PredRNN, McNet, MsNet, fRNN, PredRNN++, E3D-LSTM, Conv-TT-LSTM, LMC-Memory, V-3D-ConvLSTM, R-ST-ConvLSTM, PredRNN-V2, VPTR*, 3-LayerHVP},
        minor tick num=0,
        xticklabel style={rotate=90},
        %xlabel={year},
        %xlabel style={yshift=2mm};
        ylabel={PSNR},
        ylabel near ticks,
        legend pos=north west,
        grid,
        title={PSNR}
        ]
        \addplot table {psnr_data.txt};
      \end{axis}
\end{tikzpicture}



==> tables/configurations_table.tex <==
\begin{tabular}{lcccccc}
\hline\hline
 & \multicolumn{3}{c}{KTH ($10 \rightarrow 20$)} & \multicolumn{3}{c}{Moving MNIST ($10 \rightarrow 10$)}  \\
 \cmidrule(lr){2-4}\cmidrule(lr){5-7}
Method &  PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$  & PSNR$\uparrow$ & SSIM$\uparrow$ & MSE$\downarrow$  \\ [0.5ex]
\hline
1-layer S-HR-VQVAE$^*$  & 26.91    & 0.830  & 0.173  & 29.01  & 0.865  & 67.55\\
3-layer S-HR-VQVAE      & 28.43    & 0.863  & 0.130  & 30.35  & 0.916  & 55.46\\
9-layer S-HR-VQVAE      & 27.70    & 0.844  & 0.148  & 29.86  & 0.902  & 61.73\\
\hline
%1-layer S-HR-VQVAE$^*$  & -    & -  & -  & -  & -  & - \\
3-layer S-HR-VQVAE (joint)     & 28.49    & 0.897  & 0.093  & 31.49  & 0.919  & 46.20\\
%9-layer S-HR-VQVAE      & -    & -  & -  & -  & -  & - \\
\hline\hline
\multicolumn{7}{l}{* Equivalent to VQVAE + ST-PixelCNN}
\end{tabular}


==> tables/results_table.tex <==
\begin{tabular}{lccccccc}
\hline\hline
 & \multicolumn{3}{c}{KTH Human Action ($10 \rightarrow 20$)} & \multicolumn{3}{c}{Moving-MNIST ($10 \rightarrow 10$)} \\
 \cmidrule(lr){2-4}\cmidrule(lr){5-7}
Method &  PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$   & PSNR$\uparrow$ & SSIM$\uparrow$ & MSE$\downarrow$ & \#Params$\downarrow$ \\ [0.5ex]
\hline
ConvLSTM (2015)~\cite{shi2015convolutional}    &  23.01         & 0.704         & 0.156           & 28.38          & 0.713           & 103.3         & 16.60M\\ 
DFN (2016)~\cite{jia2016dynamic}               &  27.26         & 0.794         & $\times$        & $\times$       & 0.726           & 89.0          & $\times$ \\
CDNA (2016)~\cite{finn2016unsupervised}        &  23.75         & 0.752         & $\times$        & $\times$       & 0.728           & 97.4          & $\times$ \\
DrNet(2017)~\cite{denton2017unsupervised}      &  25.56         & 0.764         & $\times$        & 14.79          & 0.650           & $\times$      & 23.30M\\
PredRNN (2017)~\cite{wang2017predrnn}          &  27.55         & 0.839         & 0.167           & $\times$       & 0.869           & 56.8          & 23.85M\\
McNet (2018)~\cite{villegas2017decomposing}    &  25.95         & 0.804         & $\times$        & 12.53          & 0.421           & 268.7         & 3.50M \\
MsNet (2018)~\cite{lee2018mutual}              &  27.08         & 0.876         & $\times$        & $\times$       & $\times$        & $\times$      & 3.20M \\
fRNN (2018)~\cite{oliu2018folded}              &  26.12         & 0.771         & $\times$        & $\times$       & 0.819           & 69.7          & $\times$\\
PredRNN++ (2018)~\cite{wang2018predrnn++}      &  28.62         & 0.888         & 0.229           & $\times$       & 0.885           & 47.9          & 15.40M\\
E3D-LSTM (2019)~\cite{wang2019eidetic}         &  27.92         & 0.893         & $\times$        & $\times$       & 0.910           & 44.2          & 41.94M \\
MIM (2019)~\cite{wang2019memory}               &  $\times$      & $\times$      & $\times$        & $\times$       & 0.874           & 52.0          & 37.37M\\
Conv-TT-LSTM (2020)~\cite{su2020convolutional} & 28.36          & 0.907         & 0.133           & $\times$       & 0.924           & 53.0          & 2.69M\\
PhyDNet (2020)~\cite{guen2020disentangling}    & 28.69          &   $\times$    &  0.188          & $\times$       & 0.947           & 24.4          & 3.10M\\
Jin et al. (2020)~\cite{jin2020exploring}      & 29.85          &  0.893        & 0.118           & $\times$       & $\times$        & $\times$      & $\times$\\
LMC-Memory (2021)~\cite{lee2021video}          & 28.61          & 0.894         & 0.133           & $\times$       & 0.924           & 41.5          & $\times$\\
V-3D-ConvLSTM (2021)~\cite{razali2021log}      & 28.31          & 0.866         & $\times$        & $\times$       & 0.896           & 39.4          & 12.90M \\
R-ST-ConvLSTM (2022)~\cite{saideni2022novel}   & 28.99          & 0.854         & $\times$        & 32.52          & 0.895           & $\times$      & $\times$\\
SimVP (2022)~\cite{gao2022simvp}               & 33.72          & 0.905         & $\times$        & $\times$       & 0.948           &  23.8         & 22.30M \\
PredRNN-V2 (2023)~\cite{wang2022predrnn}       & 28.37          & 0.838         & 0.139           & $\times$       & 0.891           & 48.4          & 23.86M\\
VPTR (2023)~\cite{ye2023video}                 & 26.96          & 0.879         & 0.076           & $\times$       & 0.882           & 63.6          & 162.48M\\
NPVP (2023)~\cite{ye2023unified}\scalebox{1.25}{$^*$}               & 27.66          & 0.909         & 0.066           &  28.11         & 0.958     &  $\times$   & $\times$\\
\hline
S-HR-VQVAE-disjoint (ours)   &   28.43   & 0.863  & 0.130  & 30.35 & 0.916 & 55.5 & 1.14M \\
S-HR-VQVAE-joint (ours)      &   28.49   & 0.910  & 0.093  & 31.49 & 0.919 & 46.2 & 1.14M \\

\hline\hline
\multicolumn{8}{l}{($\uparrow$) means higher is better and ($\downarrow$) means lower is better. \scalebox{1.25}{$^*$} NPVP resized KTH samples to $64\times64$ instead of standard $128\times128$.}
\end{tabular}





==> tables/results_table4.tex <==
\begin{tabular}{lccc}
\hline\hline
 & \multicolumn{3}{c}{Kitti ($5 \rightarrow 5$)}  \\
 \cmidrule(lr){2-4}
Method &  SSIM $\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$ \\ [0.5ex]
\hline
PhyDNet (2020)~\cite{guen2020disentangling}   &  0.674    &  0.403   &  19.159    \\
LMC-Memory (2021)~\cite{lee2021video}         &  0.660    &  0.410   &  18.692    \\
MotionRNN (2021)~\cite{wu2021motionrnn}       &  0.652    &  0.384   &  18.931    \\
MIMO (2023)~\cite{ning2023mimo}               &  0.703    &  0.308   &  19.616    \\
\hline

S-HR-VQVAE-joint (ours)      &     &   &   \\
\hline\hline
\multicolumn{4}{l}{($\uparrow$) means higher is better and ($\downarrow$) means lower is better.}
\end{tabular}
